Frequency Response Analysis for Reset Control Systems: Application to Predict Precision of Motion Systems

The frequency response analysis describes the steady-state responses of a system to sinusoidal inputs at different frequencies, providing control engineers with an effective tool for designing control systems in the frequency domain. However, conducting this analysis for closed-loop reset systems is challenging due to system nonlinearity. This paper addresses this challenge through two key contributions. First, it introduces novel analysis methods for both open-loop and closed-loop reset control systems at steady states. These methods decompose the frequency responses of reset systems into base-linear and nonlinear components. Second, building upon this analysis, the paper develops closed-loop higher-order sinusoidal-input describing functions for reset control systems at steady states. These functions facilitate the analysis of frequency-domain properties, establish a connection between open-loop and closed-loop analysis, and enable the prediction of time-domain performance for reset systems. The accuracy and effectiveness of the proposed methods are successfully validated through simulations and experiments conducted on a reset Proportional-Integral-Derivative (PID) controlled precision motion system.

==> appen.tex <==

\section{True first reset instant}

\subsubsection{Model for multiple reset systems}
\begin{rem}
	Suppose $p_i, \ i \in \mathbb{N}^k$ is the pole of $\mathcal{S}_{bl}(\omega)$, with $k$ being the number of the poles. Similarly, $q_i, \ i \in \mathbb{N}^m$ is defined as the pole of $\mathcal{T}_{bl}(\omega)$, with $m$ being the number of its poles. Then $\mathcal{S}_{bl}(\omega)$ and $\mathcal{T}_{bl}(\omega)$ can be represented by
	\begin{equation}
		\label{eq: Sbl1,Tbl1}
		\begin{aligned}
			\mathcal{S}_{bl}(\omega) &= {S}_{bl}(\omega)\prod_{i=1}^{i=k}\frac{j\omega-p_i}{j\omega-p_i},\\
			\mathcal{T}_{bl}(\omega) &= {T}_{bl}(\omega)\prod_{i=1}^{i=m}\frac{j\omega-q_i}{j\omega-q_i},
		\end{aligned}
	\end{equation}
	where $\omega$ is an arbitrary angular frequency.
\end{rem}
\begin{lem}
	In time-domain, the transient and steady-state responses of error $e_{bl}(t)$ and output $y_{bl}(t)$ of base-linear $\mathcal{RCS}$ in closed-loop with respect to the a sinusoidal input signal $r(t) = A\sin (\omega t)$ whose Fourier transform is $R(\omega) = \mathscr{F}[r(t)]$ are given by
	\begin{equation}
		\label{eq: ebl}
		\begin{aligned}
			e_{bl}(t) &= e_{blss}(t) + e_{blts}(t),\\
			e_{blss}(t) &= A|\mathcal{S}_{bl}(\omega)|\sin \left[ \omega t+ \angle \mathcal{S}_{bl}(\omega)\right] ,\\
			e_{blts}(t) &= - A|\mathcal{S}_{bl}(\omega)|\sum_{i=1}^{i=k}e^{p_i t} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right),
		\end{aligned}
	\end{equation}
and
	\begin{equation}
		\label{eq: ybl}
		\begin{aligned}
			y_{bl}(t) &= y_{blss}(t) + y_{blts}(t),\\
			y_{blss}(t) &= A|\mathcal{T}_{bl}(\omega)|\sin \left[ \omega t+ \angle \mathcal{T}_{bl}(\omega)\right] ,\\
			y_{blts}(t) &= -A|\mathcal{T}_{bl}(\omega)| \sum_{i=1}^{i=m}e^{q_i t} \sin \left( \angle \mathcal{T}_{bl}(\omega)\right),
		\end{aligned}
	\end{equation}
where $e_{blss}(t)$ and $y_{blss}(t)$, $e_{blts}(t)$ and $y_{blts}(t)$ are the steady-state responses and transient-state responses of $e_{bl}(t)$ and $y_{bl}(t)$ respectively.
\end{lem}

\begin{pf}
	For an exponential input signal $r_e(t) = e^{j\omega t}$ whose Fourier transform is $R_e(\omega) = \mathscr{F}[r_e(t)]=\frac{1}{j\omega-j\omega}$, the error $E_{bl}(\omega)$ and output $Y_{bl}(\omega)$ of base-linear $\mathcal{RCS}$ are given by
	\begin{equation}
		\begin{aligned}
			E_{bl}(\omega) &= R_e(\omega)S_{bl}(\omega) &= \frac{S_{bl}(\omega)}{j\omega-j\omega},\\
			Y_{bl}(\omega) &= R_e(\omega)T_{bl}(\omega) &= \frac{T_{bl}(\omega)}{j\omega-j\omega}.	
		\end{aligned}
	\end{equation}
	
	From \eqref{eq: Sbl1,Tbl1}, $E_{bl}(\omega)$ and $Y_{bl}(\omega)$ can be given by
	\begin{equation}
		\begin{aligned}
			E_{bl}(\omega) &= \frac{\mathcal{S}_{bl}(\omega)}{j\omega-j\omega} - \sum_{i=1}^{i=k}\frac{\mathcal{S}_{bl}(\omega)}{j\omega-p_i},\\
			Y_{bl}(j\omega) &= \frac{\mathcal{T}_{bl}(\omega)}{j\omega-j\omega} - \sum_{i=1}^{i=m}\frac{\mathcal{T}_{bl}(\omega)}{j\omega-q_i}.
		\end{aligned}
	\end{equation}
	
	$e_{blss}(t)$ and $e_{blts}(t)$ are the steady-state response and transient-state response of $e_{bl}(t)$ which are given by
	\begin{equation}
		\begin{aligned}
			e_{bl}(t) &= e_{blss}(t) + e_{blts}(t),\\
			e_{blss}(t) &= \mathscr{F}^{-1}\left[ \frac{\mathcal{S}_{bl}(\omega)}{j\omega-j\omega}\right]  = e^{j\left[ \omega t+\mathcal{S}_{bl}(\omega)\right] } ,\\
			e_{blts}(t) &= \mathscr{F}^{-1}\left[ - \sum_{i=1}^{i=k}\frac{\mathcal{S}_{bl}(\omega)}{j\omega-p_i}\right] = -\sum_{i=1}^{i=k}e^{p_i t} e^{j\mathcal{S}_{bl}(\omega)}.
		\end{aligned}
	\end{equation}

	Based on the \enquote{\emph{Euler Formula}}, for a sinusoidal input signal $r(t) = A\sin (\omega t)$ whose Fourier transform is $R(\omega) = \mathscr{F}[r(t)]$, the steady-state response $e_{blss}(t)$ and transient-state response $e_{blts}(t)$ of error signal $e_{bl}(t)$ are given by
	\begin{equation}
	\label{eq: ebl}
		\begin{aligned}
			e_{bl}(t) &= e_{blss}(t) + e_{blts}(t),\\
			e_{blss}(t) &= A|\mathcal{S}_{bl}(\omega)|\sin \left[ \omega t+ \angle \mathcal{S}_{bl}(\omega)\right] ,\\
			e_{blts}(t) &= - A|\mathcal{S}_{bl}(\omega)|\sum_{i=1}^{i=k}e^{p_i t} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right).
		\end{aligned}
	\end{equation}
	
	The steady-state response $y_{blss}(t)$ and transient-state response $y_{blts}(t)$ of output signal $y_{bl}(t)$ in \eqref{eq: ybl} can be derived as the same process as above.
\end{pf}

\begin{lem}
	For a sinusoidal input signal $r(t) = A\sin (\omega t)$, the first reset instant $t_1 \in t_R$ of $\mathcal{RCS}$ is the solution of 
	\begin{equation}
		\label{eq: t1}
		\sin \left[ \omega t_1+ \angle \mathcal{S}_{bl}(\omega)\right]=  \sum_{i=1}^{i=k}e^{p_i t_1} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right).
	\end{equation}
\end{lem}
\begin{pf}
	The first reset action appears at when the base-linear error signal denoted by $e_{bl}(t)$ hits to zero. $e_{bl}(t)$ is given by \eqref{eq: ebl}, then the first solution of $e_{bl}(t_1) = 0$ is shown in \eqref{eq: t1}.
\end{pf}
Thus, 
\begin{equation}
    \sin \left[ \omega t_1+ \angle \mathcal{S}_{bl}(\omega)\right] = \sum_{i=1}^{i=k}e^{p_i t_1} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right) <1,
\end{equation}
thus, 
\begin{equation}
    e_{bl}''(t_1) >0.
\end{equation}
